Characterizing Pulsars Detected in the Rapid ASKAP Continuum Survey

We present the detection of 661 known pulsars observed with the Australian SKA Pathfinder (ASKAP) telescope at 888 MHz as a part of the Rapid ASKAP Continuum Survey (RACS). Detections were made through astrometric coincidence and we estimate the false alarm rate of our sample to be ~0.5%. Using archival data at 400 and 1400 MHz, we estimate the power law spectral indices for the pulsars in our sample and find that the mean spectral index is -1.78 +/- 0.6. However, we also find that a single power law is inadequate to model all the observed spectra. With the addition of the flux densities between 150 MHz and 3 GHz from various imaging surveys, we find that up to 40% of our sample shows deviations from a simple power law model. Using Stokes V measurements from the RACS data, we measured the circular polarization fraction for 9% of our sample and find that the mean polarization fraction is ~10% (consistent between detections and upper limits). Using the dispersion measure (DM) derived distance we estimate the pseudo luminosity of the pulsars and do not find any strong evidence for a correlation with the pulsars' intrinsic properties.

==> megan_pulsartable.tex <==
\begin{deluxetable*}{lcccccccccccc}\label{tbl:}
\tabletypesize{\footnotesize}
%\begin{center}
%\small
\tablecaption{\fixme{Megan will replace with table of Stokes V detections}}
\tablewidth{0pt}
\tablehead{
%& \multicolumn{5}{c|}{PSRCAT} &  \multicolumn{6}{c}{RACS} \\
PSR & \colhead{S$_{400}$} & S$_{1400}$ & S$_{888;\rm{calc}}$ & S$_{\rm RACSI}$ & S$_{\rm RACSV}$  & $\alpha$\\
&  (mJy) & (mJy) & (mJy) & (mJy) & (mJy)
}
\startdata
J0034$-$0721 & 52 $\pm$ 12 & 1.6 $\pm$ 0.3 & 19 $\pm$ 3 & 4.69 $\pm$ 0.06 & $<$ 0.5772 & $-$1.2 $\pm$ 0.2 &  \doubleslash 
J0038$-$2501 & 11 $\pm$ 2 & 0.9 $\pm$ 0.2 & 5 $\pm$ 4 & 12.1 $\pm$ 0.07 & $<$ 0.6047 & $-$2.5 $\pm$ 0.3 &  \doubleslash 
J0134$-$2937 & 38 $\pm$ 15 & 1.2 $\pm$ 0.2 & 3 $\pm$ 4 & 5.71 $\pm$ 0.05 & $<$ 0.8091 & $-$2.9 $\pm$ 0.2 &  \doubleslash 
J0151$-$0635 & 34 $\pm$ 7 & 1.7 $\pm$ 0.3 & 2.7 $\pm$ 1.0 & 4.51 $\pm$ 0.07 & $<$ 0.5978 & $-$1.8 $\pm$ 0.1 &  \doubleslash 
J0211$-$8159 & 82 $\pm$ 10 & 2.6 $\pm$ 0.5 & 29 $\pm$ 5 & 56.1 $\pm$ 0.1 & $<$ 0.7182 & $-$1.3 $\pm$ 0.2 &  \doubleslash 
\\
J0255$-$5304 & 16 $\pm$ 3 & 3.2 $\pm$ 0.4 & 4 $\pm$ 1 & 4.36 $\pm$ 0.05 & $<$ 0.7427 & $-$1.9 $\pm$ 0.1 &  \doubleslash 
J0302+2252 & 19 $\pm$ 0.9 & 2.7 $\pm$ 0.2 & 3.2 $\pm$ 0.2 & 5.08 $\pm$ 0.08 & $<$ 0.5794 & $-$1.17 $\pm$ 0.04 &  \doubleslash
J0323+3944 & 8 $\pm$ 0.2 & 1.9 $\pm$ 0.5 & 5 $\pm$ 1 & 6.2 $\pm$ 0.05 & $<$ 0.6859 & $-$1.7 $\pm$ 0.1 &  \doubleslash 
J0337+1715 & 22 $\pm$ 0.9 & 0.6 $\pm$ 0.3 & 7 $\pm$ 1 & 7.9 $\pm$ 0.04 & $<$ 0.7429 & $-$1.8 $\pm$ 0.1 &  \doubleslash 
J0343$-$3000 & 31 $\pm$ 2 & 2.6 $\pm$ 0.8 & 3.7 $\pm$ 0.3 & 2.79 $\pm$ 0.02 & $<$ 0.694 & $-$0.7 $\pm$ 0.09 &  \doubleslash 
\\
J0348+0432 & 6 $\pm$ 0.6 & 1.8 $\pm$ 0.3 & 3.6 $\pm$ 0.9 & 4.97 $\pm$ 0.04 & $<$ 1.0391 & $-$1.4 $\pm$ 0.2 &  \doubleslash 
J0401$-$7608 & 11 $\pm$ 0.7 & 2.3 $\pm$ 0.9 & 1 $\pm$ 2 & 3.83 $\pm$ 0.03 & $<$ 0.502 & $-$2.1 $\pm$ 0.4 &  \doubleslash 
J0407+1607 & 8 $\pm$ 0.6 & 2.74 $\pm$ 0.04 & 4.0 $\pm$ 0.7 & 2.63 $\pm$ 0.03 & $<$ 0.7573 & $-$0.9 $\pm$ 0.2 &  \doubleslash 
J0435+2749 & 30 $\pm$ 5 & 1.7 $\pm$ 0.4 & 8 $\pm$ 4 & 4.88 $\pm$ 0.04 & $<$ 0.6888 & $-$1.6 $\pm$ 0.4 &  \doubleslash 
J0450$-$1248 & 4 $\pm$ 2 & 1.2 $\pm$ 0.3 & 14 $\pm$ 3 & 13.48 $\pm$ 0.09 & $<$ 0.8157 & $-$2.3 $\pm$ 0.2 &  \doubleslash 
\\
J0452$-$1759 & 89 $\pm$ 14 & 0.28 $\pm$ 0.07 & 6 $\pm$ 1 & 46.2 $\pm$ 0.1 & $<$ 0.6142 & $-$1.1 $\pm$ 0.2 &  \doubleslash 
J0509+0856 & 4 $\pm$ 2 & 0.8 $\pm$ 0.3 & 22 $\pm$ 1 & 4.12 $\pm$ 0.04 & $<$ 0.7524 & $-$0.27 $\pm$ 0.09 &  \doubleslash 
J0517+2212 & 28 $\pm$ 3 & 5.9 $\pm$ 0.9 & 3 $\pm$ 1 & 1.34 $\pm$ 0.03 & $<$ 0.6465 & $-$1.7 $\pm$ 0.2 &  \doubleslash 
J0525+1115 & 15 $\pm$ 2 & 2.0 $\pm$ 0.7 & 5 $\pm$ 3 & 8.4 $\pm$ 0.07 & $<$ 0.7377 & $-$2.0 $\pm$ 0.3 &  \doubleslash 
J0537$-$6910 & 28 $\pm$ 6 & 3.8 $\pm$ 0.8 & 5.1 $\pm$ 0.6 & 5.31 $\pm$ 0.09 & $<$ 0.5969 & $-$1.4 $\pm$ 0.1 &  \doubleslash 
\enddata
\tablecomments{Measured fluxes from the literature as well as this paper. Columns show the fluxes at 400 and 1400\,MHz (taken from PSRCAT), the predicted flux at 888\,MHz, the measured flux at 888\,MHz for Stokes I, the upper limit on flux for Stokes V, and the fit spectral index $\alpha$ using these 3 frequencies. 
}  
\end{deluxetable*}

==> msps.tex <==
\begin{deluxetable*}{lcccccccccccc}\label{tbl:msps}
\tabletypesize{\small}
%\begin{center}
%\small
\tablecaption{Millisecond pulsars with measurable spectral indices}
\tablewidth{0pt}
\tablehead{
%& \multicolumn{5}{c|}{PSRCAT} &  \multicolumn{6}{c}{RACS} \\
PSR & \colhead{S$_{400}$} & S$_{1400}$ & S$_{\rm RACSI}$ & S$_{\rm RACSV}$  & $\alpha$\\
&  (mJy) & (mJy) & (mJy) & (mJy) &
}
\startdata
%J0509+0856 & 5.0 $\pm$ 0.0 & 0.8 $\pm$ 0.0 & 5.39 $\pm$ 0.05 & $<$0.8256 & $-$1.46 $\pm$ 0.11 \doubleslash
%J0621+1002 & 9.5 $\pm$ 0.0 & 1.9 $\pm$ 0.3 & 4.41 $\pm$ 0.04 & $<$0.7703 & $-$1.28 $\pm$ 0.14 \doubleslash
%J0751+1807 & 10.0 $\pm$ 0.0 & 3.2 $\pm$ 0.7 & 2.13 $\pm$ 0.04 & $<$0.5278 & $-$0.91 $\pm$ 0.17 \doubleslash
J1045$-$4509 & 15 $\pm$ 3 & 2.74 $\pm$ 0.04 & \phantom{0}8.4 $\pm$ \fixme{0.07} & $<$0.6 & $-$1.4 $\pm$ 0.1 \doubleslash
%J1300+1240 & 20.0 $\pm$ 0.0 & 2.0 $\pm$ 1.0 & 1.47 $\pm$ 0.03 & $<$0.6441 & $-$1.84 $\pm$ 0.36 \doubleslash
J1603$-$7202 & 21 $\pm$ 2 & 3.5 $\pm$ 0.2 & 9.57 $\pm$ 0.04 & $<$0.5 & $-$1.43 $\pm$ 0.09 \doubleslash
%J1722$-$3712 & 25.0 $\pm$ 0.0 & 3.8 $\pm$ 0.3 & 9.21 $\pm$ 0.15 & $<$1.0476 & $-$1.5 $\pm$ 0.1 \doubleslash
%J1817$-$3618 & 22.0 $\pm$ 0.0 & 3.2 $\pm$ 0.6 & 7.62 $\pm$ 0.05 & $<$1.3936 & $-$1.54 $\pm$ 0.16 \doubleslash
J1823+0550 & 18 $\pm$ 2 & 1.7 $\pm$ 0.4 & 13.17 $\pm$ 0.04\phantom{0} & $<$0.6 & $-$1.9 $\pm$ 0.2 \doubleslash
J1847$-$0402 & 75 $\pm$ 3 & 4.9 $\pm$ 0.3 & 10.76 $\pm$ 0.08\phantom{0} & $<$1.2 & $-$2.18 $\pm$ 0.06 \doubleslash
J1901+0331 & 165 $\pm$ 10 & 4.2 $\pm$ 0.4 & 11.5 $\pm$ 0.2\phantom{0} & $<$1.0 & $-$2.93 $\pm$ 0.09 \doubleslash \\
%J1904+0004 & 16.0 $\pm$ 0.0 & 2.9 $\pm$ 0.6 & 14.71 $\pm$ 0.06 & $<$1.2093 & $-$1.36 $\pm$ 0.17 \doubleslash
J1937+2544 & \phantom{0}6.6 $\pm$ 0.4 & 1.4 $\pm$ 0.3 & 8.84 $\pm$ 0.08 & $<$0.6 & $-$1.2 $\pm$ 0.2 \doubleslash
J2006$-$0807 & 20 $\pm$ 3 & 4.7 $\pm$ 0.9 & 7.0 $\pm$ 0.1 & $<$0.6 & $-$1.2 $\pm$ 0.2 \doubleslash
J2055+3630 & 28 $\pm$ 1 & 2.6 $\pm$ 0.1 & 8.20 $\pm$ 0.06 & $<$0.5 & $-$1.90 $\pm$ 0.04 \doubleslash
J2124$-$3358 & 17 $\pm$ 4 & 4.5 $\pm$ 0.2 & 5.91 $\pm$ 0.07 & $<$0.7 & $-$1.1 $\pm$ 0.2 \doubleslash
J2157+4017 & 105 $\pm$ 7\phantom{0} & 17 $\pm$ 2\phantom{0} & 52.4 $\pm$ 0.1\phantom{0} & $<$1.0 & $-$1.5 $\pm$ 0.1 \doubleslash \\
J0922+0638 & 52 $\pm$ 6 & 10 $\pm$ 3\phantom{0} & 39.2 $\pm$ 0.2\phantom{0} & $<$3.3 & $-$1.3 $\pm$ 0.2 \doubleslash
%J1157$-$6224 & 145.0 $\pm$ 0.0 & 14.0 $\pm$ 3.0 & 29.57 $\pm$ 0.08 & $<$5.352 & $-$1.87 $\pm$ 0.17 \doubleslash
%J1326$-$5859 & 120.0 $\pm$ 0.0 & 18.0 $\pm$ 3.6 & 31.88 $\pm$ 0.1 & $<$3.653 & $-$1.51 $\pm$ 0.16 \doubleslash
%J1327$-$6222 & 135.0 $\pm$ 0.0 & 21.0 $\pm$ 4.2 & 65.35 $\pm$ 0.17 & $<$3.929 & $-$1.49 $\pm$ 0.16 \doubleslash
%J1359$-$6038 & 105.0 $\pm$ 0.0 & 12.5 $\pm$ 0.6 & 45.04 $\pm$ 0.13 & $<$6.465 & $-$1.7 $\pm$ 0.09 \doubleslash
%J1428$-$5530 & 35.0 $\pm$ 0.0 & 6.5 $\pm$ 1.3 & 22.45 $\pm$ 0.13 & $<$1.077 & $-$1.34 $\pm$ 0.16 \doubleslash
J1709$-$4429 & 25 $\pm$ 4 & 12.1 $\pm$ 0.7\phantom{0} & 16.54 $\pm$ 0.09\phantom{0} & $<$3.5 & $-$0.6 $\pm$ 0.1 \doubleslash
J1730$-$2304 & 43 $\pm$ 6 & 4.0 $\pm$ 0.2 & 12.64 $\pm$ 0.09\phantom{0} & $<$1.7 & $-$1.9 $\pm$ 0.1 \doubleslash
J1752$-$2806 & 1100 $\pm$ 100 & 48 $\pm$ 10 & 226 $\pm$ 2\phantom{10} & $<$3.3 & $-$2.5 $\pm$ 0.2 \doubleslash
J1917+1353 & 43 $\pm$ 3 & 7 $\pm$ 1 & 14.12 $\pm$ 0.07\phantom{0} & $<$1.5 & $-$1.5 $\pm$ 0.2 \doubleslash
\enddata
\tablecomments{Fluxes are measured in RACS Stokes I at 888\,MHz (with an upper limit on Stokes V) and from PSRCAT at 400 and 1400\,MHz. Spectral indices $\alpha$ were fit with a least-squares using these three flux measurements.  
}  
\end{deluxetable*}



==> stokesv.tex <==
\begin{deluxetable*}{lcccccccccccc}\label{tbl:stokesv}
\tabletypesize{\small}
%\begin{center}
%\small
\tablecaption{Detections in Stokes I and V with spectral index fit}
\tablewidth{0pt}
\tablehead{
%& \multicolumn{5}{c|}{PSRCAT} &  \multicolumn{6}{c}{RACS} \\
PSR & \colhead{S$_{400}$} & S$_{1400}$ & S$_{888;\rm{calc}}$ & S$_{\rm RACSI}$ & S$_{\rm RACSV}$  & $\alpha$\\
&  (mJy) & (mJy) & (mJy) & (mJy) & (mJy)
}
\startdata
%J1948+3540 & 145 $\pm$ 9 & 8.3 $\pm$ 0.9 & 23.5 $\pm$ 2.7 & 16.77 $\pm$ 0.0 & 3.831 $\pm$ 0.075 & $-$2.28 $\pm$ 0.09 &  \doubleslash 
J0304+1932 & 27 $\pm$ 3 & 15 $\pm$ 3\phantom{0} & 19 $\pm$ 3 & 8.68 $\pm$ 0.08 & 1.15 $\pm$ 0.04 & $-$0.5 $\pm$ 0.2 &  \doubleslash 
J0437$-$4715 & \phantom{0}550 $\pm$ 100 & 150 $\pm$ 2\phantom{10} & 241 $\pm$ 3 & 270.8 $\pm$ 0.5 & $-$13.6 $\pm$ $-$0.3 & $-$1.04 $\pm$ 0.03 &  \doubleslash 
J0614+2229 & 29 $\pm$ 1 & 3.3 $\pm$ 0.2 & 7.3 $\pm$ 0.5 & 9.07 $\pm$ 0.08 & 1.21 $\pm$ 0.04 & $-$1.73 $\pm$ 0.05 &  \doubleslash 
J0630$-$2834 & 206 $\pm$ 22 & 31 $\pm$ 6\phantom{0} & 63 $\pm$ 12 & 66.0 $\pm$ 0.4 & $-$3.2 $\pm$ $-$0.1 & $-$1.5 $\pm$ 0.2 &  \doubleslash 
J0711$-$6830 & 10 $\pm$ 1 & 3.7 $\pm$ 0.4 & 5.3 $\pm$ 0.6 & 25.58 $\pm$ 0.06 & $-$3.40 $\pm$ $-$0.05 & $-$0.8 $\pm$ 0.1 &  \doubleslash \\
J0742$-$2822 & 296 $\pm$ 14 & 26 $\pm$ 2\phantom{0} & 63 $\pm$ 5 & 67.0 $\pm$ 0.4 & $-$2.35 $\pm$ $-$0.04 & $-$1.94 $\pm$ 0.07 &  \doubleslash 
J0820$-$1350 & 102 $\pm$ 6\phantom{0} & 6 $\pm$ 2 & 17 $\pm$ 6 & 15.60 $\pm$ 0.07 & $-$2.72 $\pm$ $-$0.06 & $-$2.3 $\pm$ 0.2 &  \doubleslash 
J0922+0638 & 52 $\pm$ 6 & 10 $\pm$ 3\phantom{0} & 18 $\pm$ 5 & 39.2 $\pm$ 0.2 & 3.3 $\pm$ 0.1 & $-$1.3 $\pm$ 0.2 &  \doubleslash 
J0944$-$1354 & 26 $\pm$ 4 & 0.6 $\pm$ 0.2 & 2 $\pm$ 5 & 11.44 $\pm$ 0.08 & 2.17 $\pm$ 0.02 & $-$3.0 $\pm$ 0.3 &  \doubleslash 
J0953+0755 & \phantom{0}400 $\pm$ 200 & 100 $\pm$ 40\phantom{0} & 166 $\pm$ 65 & 410.9 $\pm$ 0.8 & $-$13.8 $\pm$ $-$0.1 & $-$1.1 $\pm$ 0.5 &  \doubleslash \\
J1136+1551 & 257 $\pm$ 53 & 20 $\pm$ 10 & 51 $\pm$ 25 & 26.5 $\pm$ 0.1 & $-$3.32 $\pm$ $-$0.09 & $-$2.0 $\pm$ 0.4 &  \doubleslash 
J1709$-$4429 & 25 $\pm$ 4 & 12.1 $\pm$ 0.7\phantom{0} & 15.8 $\pm$ 0.9 & 16.54 $\pm$ 0.09 & $-$3.51 $\pm$ $-$0.05 & $-$0.6 $\pm$ 0.1 &  \doubleslash 
J1730$-$2304 & 43 $\pm$ 6 & 4.0 $\pm$ 0.2 & 10 $\pm$ 1 & 12.64 $\pm$ 0.09 & $-$1.65 $\pm$ $-$0.03 & $-$1.9 $\pm$ 0.1 &  \doubleslash 
J1752$-$2806 & 1100 $\pm$ 100 & 48 $\pm$ 10 & 149 $\pm$ 30 & 226 $\pm$ 2 & 3.3 $\pm$ 0.2 & $-$2.5 $\pm$ 0.2 &  \doubleslash 
J1803$-$2137 & 23 $\pm$ 5 & 10 $\pm$ 1\phantom{0} & 13 $\pm$ 2 & 14.94 $\pm$ 0.08 & 4.02 $\pm$ 0.06 & $-$0.7 $\pm$ 0.2 &  \doubleslash \\
J1820$-$0427 & 157 $\pm$ 6\phantom{0} & 9.3 $\pm$ 1.9 & 26 $\pm$ 5 & 23.6 $\pm$ 0.1 & $-$2.19 $\pm$ $-$0.07 & $-$2.3 $\pm$ 0.1 &  \doubleslash 
J1915+1009 & 23 $\pm$ 2 & 2.0 $\pm$ 0.4 & 5 $\pm$ 2 & 5.96 $\pm$ 0.04 & 2.53 $\pm$ 0.05 & $-$2.0 $\pm$ 0.2 &  \doubleslash 
J1917+1353 & 43 $\pm$ 3 & 7 $\pm$ 1 & 13 $\pm$ 3 & 14.12 $\pm$ 0.07 & $-$1.50 $\pm$ $-$0.05 & $-$1.5 $\pm$ 0.2 &  \doubleslash 
J1932+1059 & 303 $\pm$ 76 & 29 $\pm$ 6\phantom{0} & 68 $\pm$ 14 & 243.2 $\pm$ 0.4 & $-$19.03 $\pm$ $-$0.09 & $-$1.9 $\pm$ 0.3 &  \doubleslash 
J1935+1616 & 242 $\pm$ 22 & 58 $\pm$ 1\phantom{0} & 98 $\pm$ 2 & 138.3 $\pm$ 0.2 & 1.49 $\pm$ 0.03 & $-$1.14 $\pm$ 0.05 &  \doubleslash \\
J2018+2839 & 314 $\pm$ 30 & 30 $\pm$ 13 & 70 $\pm$ 28 & 45 $\pm$ 1 & $-$4.15 $\pm$ $-$0.07 & $-$1.9 $\pm$ 0.3 &  \doubleslash 
%J2022+2854 & 71 $\pm$ 7.0 & 38.0 $\pm$ 0.0 & 47.69 $\pm$ 4.15 & 53.27 $\pm$ 0.17 & $-$6.49 $\pm$ $-$0.103 & $-$0.5 $\pm$ 0.1 &  \doubleslash 
J2048$-$1616 & 116 $\pm$ 26 & 22 $\pm$ 4\phantom{0} & 40 $\pm$ 8 & 55.3 $\pm$ 0.1 & 3.35 $\pm$ 0.04 & $-$1.3 $\pm$ 0.2 &  \doubleslash 
\enddata
\tablecomments{Measured fluxes from the literature as well as this paper. Columns show the fluxes at 400 and 1400\,MHz (taken from PSRCAT), the predicted flux at 888\,MHz, the measured flux at 888\,MHz for Stokes I, the upper limit on flux for Stokes V, and the fit spectral index $\alpha$ using these 3 frequencies. 
}  
\end{deluxetable*}

